An Analysis of COVID-19 Knowledge Graph Construction and Applications

The construction and application of knowledge graphs have seen a rapid increase across many disciplines in recent years. Additionally, the problem of uncovering relationships between developments in the COVID-19 pandemic and social media behavior is of great interest to researchers hoping to curb the spread of the disease. In this paper we present a knowledge graph constructed from COVID-19 related tweets in the Los Angeles area, supplemented with federal and state policy announcements and disease spread statistics. By incorporating dates, topics, and events as entities, we construct a knowledge graph that describes the connections between these useful information. We use natural language processing and change point analysis to extract tweet-topic, tweet-date, and event-date relations. Further analysis on the constructed knowledge graph provides insight into how tweets reflect public sentiments towards COVID-19 related topics and how changes in these sentiments correlate with real-world events.

==> UCLA REU KG 10 Pages Report/abstract.tex <==
\begin{abstract}
%The construction and application of knowledge graphs have seen a rapid increase across many disciplines in recent years. Additionally, the problem of uncovering relationships between developments in the COVID-19 pandemic and social media behavior is of great interest to researchers hoping to curb the spread of the disease. In the following paper we present a knowledge base constructed from COVID-19 related tweets and apply it to better understand the interaction between social media discourse, public policy and disease spread. We supplement the social network of tweets with external information, temporal data and thematic classification, and represent the underlying relationships between these entities. Using methods from natural language processing, change point analysis, topic modelling, graph embedding and network theory, we gain insight into the flow of COVID-19 sentiment over Twitter, popular topics, and communities formed on Twitter during the pandemic. By applying various graph-based analysis techniques, we have a better understanding of the structure and relations inside our knowledge graph, and how the graph interprets the real world.

% The past decade has seen a rapid increase in Knowledge Graph construction and analysis due to its vast industrial and academic applications \cite{Zou_2020}. To answer questions related to the spread of COVID-19 and the evolution of the sentiment of people in relation to COVID-19, we construct a knowledge graph using Twitter data from Los Angeles, as well as federal and state policy announcements, and disease spread statistics. We supplement our graph with dates, topics and events as entities as well as keyword-tweet, tweet-topic, tweet-date, and  event-date relations that were extracted using natural language methods and change point analysis. Through our analysis, we conclude that public opinions on Twitter closely reflects real-world events and thus we infer that opinions and other information from social media are strongly connected with real-world events.

The construction and application of knowledge graphs have seen a rapid increase across many disciplines in recent years. Additionally, the problem of uncovering relationships between developments in the COVID-19 pandemic and social media behavior is of great interest to researchers hoping to curb the spread of the disease. In this paper we present a knowledge graph constructed from COVID-19 related tweets in the Los Angeles area, supplemented with federal and state policy announcements and disease spread statistics. By incorporating dates, topics, and events as entities, we construct a knowledge graph that describes the connections between these useful information. We use natural language processing and change point analysis to extract tweet-topic, tweet-date, and event-date relations. Further analysis on the constructed knowledge graph provides insight into how tweets reflect public sentiments towards COVID-19 related topics and how changes in these sentiments correlate with real-world events.

\end{abstract}

==> UCLA REU KG 10 Pages Report/acknowledgements.tex <==
% \section{Acknowledgements}
% %We would like to thank our mentors Prof. Andrea Bertozzi, Prof. P. Jeffrey Brantingham, Prof. Junyuan (Joanne) Lin and Dr. Rishi Sonthalia for their guidance, leadership, and insight throughout the program. 
% We want to thank Prof. Deanna Needell for discussing her work on topic modelling with us,
% the 2021 CAM REU GRYD and Scientific Fields groups for their helpful collaboration and exchange of ideas, the 2020 CAM REU Knowledge Graph group for providing a foundation of knowledge graph ideas to explore, and Thomas Tu for discussing his work on subgraph matching and its applications to knowledge graphs with us.


==> UCLA REU KG 10 Pages Report/alt-intro.tex <==
\section{Introduction}

\begin{figure*}
    \centering
    \includegraphics[width = 0.8\linewidth]{KG_Construction-updated.png}
    \caption{General structure of knowledge graph with an underlying social network of tweets at the center and external information and tweet attributes surrounding the network, where dashed edges indicate an edge weighting $w$. The tweet, hashtag and user entities are objects on extracted from Twitter; and the topic and keyword entities are generated by the NMF topic model. Event entities are complied from various news sources and reflect local and federal COVID-19 policy announcements, guideline updates, case count milestones and vaccination news. Each day spanned by the dataset is represented as a date entity.}
    \label{fig:KG structure}
\end{figure*}


% This paragraph answers the question what is a knowledge graph. 
The past decade has seen a rapid increase in Knowledge Graph construction and analysis due to its vast industrial and scientific applications \cite{Zou_2020}. Knowledge graphs use a directed graph structure to store and represent semantically structured information, granting it many unique strengths over other methods of data representation. Researchers can analyze relations between data, manipulate and expand the database with ease, and quickly perform navigational operations. Nodes in the graph represent objects and often store auxiliary attributes about them, and edges represent relations between objects. Moreover, techniques exist to embed the structure in vector spaces, allowing semantic analysis, knowledge classification and conventional graph learning methods. For a detailed description of common knowledge graph practices, applications and techniques, see \cite{Zou_2020, Hogan2020, Ji2020}. A well-known knowledge graph is the Google Knowledge Graph \cite{Singhal}. Other notable examples are DBpedia\cite{Lehmann}, Freebase \cite{Bollacker2007}, Wikidata \cite{Vrande2014} and YAGO \cite{Suchanek}, large open source databases of public data. 

% \subsection{Motivation}

%These two paragraphs answers the questions what did we do and why did we do it. 
To answer questions related to the spread of COVID-19 and the evolution of the sentiment of people in relation to COVID-19, we construct a knowledge graph using Twitter data from Los Angeles, as well as federal and state policy announcements, and disease spread statistics.\footnote{https://github.com/dominicflocco/Twitter-COVID-19-Knowledge-Graph} Since the onset of the novel coronavirus pandemic, researchers from a breadth of academic disciplines have been interested in tracking the interaction between developments in the pandemic and social media use. Specifically, they would like to understand the interaction between world events, COVID-19 policy announcements, and the sentiment of people. 
A knowledge graph is well-suited for this task, as it can accurately represent the content of social media data and news announcements while preserving the underlying structure of the social network and the relationships between entities. 

Our analysis of this dataset shows that public opinions on Twitter closely reflects real-world events suggesting that content on social media is strongly connected to real-world events. By topic modelling, we extract hotly discussed topics on Twitter with associated keywords. Through sentiment analysis and change point detection, we relate temporal changes in the sentiment in each topic with important dates of real-world events. By incorporating COVID-19 policies, world events, tweets, topics, and other entities into the graph, and using edges to represent their immediate relations, one can detect relations between any two entities through a walk in the graph. We can use node similarity to examine how closely two entities are related, and link prediction to predict or negate the existence of a relation between two entities. We also classify the topics into groups through community detection. Thus, we are able to relate topics that are frequently mentioned at the same time or by same group of users. 


% This paragraph details issues with previuous work. 
The recent work TweetsCov19 \cite{Dimitrov2020} also compiles Twitter data into a knowledge graph to understand the spread of COVID-19 with some limitations. Specifically, it does not include topic modelling, policy data, and diseases statistics. Additionally, our knowledge graphs contains more recent Twitter data, reflecting newer developments in the pandemic such as vaccines and variants. There are other knowledge graphs that do not use social media data to  analyze trends in academic research related to the coronavirus pandemic, such as \cite{Domingo2020}, \cite{Michel2020} and \cite{Wang2020}. 
Additionally, recent work uses social media data to model Twitter discourse \cite{Wicke2021, Tsao2021, sha2020dynamic}, to understand public sentiment \cite{Feras2020, Lyu2021}, and to perform thematic analysis\cite{Thelwall2020}. However, such work does not use a knowledge graph structure. 


% It also lends itself to information extraction, community detection, and knowledge classification. We hope our graph can help shed light on how public policy announcements surrounding COVID-19 are received by the public, and how they impact the spread of the virus. Specifically, our research is motivated by the following questions: Can we extract major pandemic-related topics and find nuanced relationships between them? What is the interaction between world events, COVID-19 policy announcements, and Twitter sentiment? How does sentiment surrounding COVID-19 evolve, and how in turn does it correlate to the spread of the disease? Can we meaningfully cluster topics, users, tweets, and keywords; and what insight can this provide about public opinion in social media?

% This paper outlines the construction and analysis of a COVID-19 knowledge graph with many applications. The goal of the graph is to accurately model the interaction between news developments, public opinion patterns, and the spread of the virus. By combining social media data, federal and state policies, and disease statistics into the same data structure, we can analyze the relationship between these entities and effectively draw conclusions. Moreover, we employ natural language processing techniques on social media data to enrich the information stored in the structure, enabling comparison and classification of social media interactions. The construction and analysis of the graph has four parts, as outlined in Figure \ref{fig:process}: (1) filtering and cleaning the dataset, (2) extracting entities and relations through various natural language processing techniques, (3) constructing and visualizing and (4) analysing the graph. At the center of the knowledge graph is an underlying social network of tweets, which models the flow of conversation on the Twitter platform. Surrounding the social network is auxiliary information extracted from the social media data, classifications obtained through natural language processing and real-world data. We present the general structure of the graph in Figure \ref{fig:KG structure}, and provide the code and data on Github\footnote{https://github.com/dominicflocco/Twitter-COVID-19-Knowledge-Graph}. The methods of construction and analysis are explained in the following sections. 



% Our graph differs from TweetsCOV19 in several important ways. First, the tweets in our graph are specifically from Los Angeles-related accounts. Second, our graph covers a more recent timespan than TweetsCOV19. Third, our graph captures some different information than TweetsCOV19, such as sentiment changepoints for tweet topics. Fourth, we estimate tweet sentiment using VADER, while TweetsCOV19 estimates tweet sentiment with SentiStrength. Fifth, we used a larger list of keywords when searching for COVID-related tweets than TweetsCOV19 does.



\subsection{Notation}
We define a knowledge graph as a weighted and directed edge-labelled graph $G = (E,R,\Delta)$, where $E$ is a set of entities that represent the set of nodes, $R$ is a set of relation types that dictate edge labels, and $\Delta\subset E\times E\times R\times\R$. Every triple in $\Delta$ is a positive fact, denoted as $\xi=(h,t,r,w)\in\Delta$, where $h\in E$ and $t\in E$ are the head and tail nodes of the fact, $r\in R$ is the edge type that connects them, and $w$ is the weight of the edge. When the weight is unnecessary, we sometimes only write $(h,t,r)$ for an edge. The graph therefore has $n = |E|$ vertices, $|\Delta|$ edges, and $|R|$ relation types.

==> UCLA REU KG 10 Pages Report/applications.tex <==
\section{Graph Applications}

\subsection{Community Detection}
We are interested in detecting communities and comparing their behavior. 
Every user or tweet is uniquely classified to one community, and the knowledge graph is divided into 31 communities, among which there are about 10 large communities. Each large community has over 70,000 tweets and 8,000 users. The 100 NMF topics are also assigned to different communities. We find that some topics are consistently grouped together into one community, similar to semantic grouping, although we did not apply any semantic analysis here. It also implies some latent relations between topics. As listed in Table \ref{tab:communities}, topics inside some communities can be summarized as a coherent, aggregated general topic.

By observing dense connections in the knowledge graph, we can detect communities in the Twitter communication network. In some communities, we find distinct popular topics being discussed during the pandemic. We also see mixed topics in some communities. For example, in the community with aggregated topic ``holidays'' and ``traveling,'' ``stimulus check'' is also discussed. We speculate that topics related to different keywords yet grouped into the same community might have hidden relations, which is worth investigation.

We used one of the most common community detection methods called the Louvain algorithm, detailed in \cite{Campigottto2014}, which is typically applied to undirected, unweighted graphs based on modularity optimization. Focusing on maximizing the density of edges inside each community, we apply the algorithm to our knowledge graph while temporarily ignoring the edge weights, edge directions, and relation types. 

\begin{table}[htbp]
    \centering
    \caption{Topics Inside Selected Communities}
    \begin{tabular}{|p{0.85cm}|p{2.cm}|p{2.1cm}|p{2.1cm}|}
    \hline
         \textbf{Comm.}  & \textbf{Number of Tweets} &  \textbf{Number of Users} &  \textbf{Aggregated Topic}\\ 
    \hline
         1  &72515 &13755 &covid policies 
 \\ \hline
         2&71805&8957&hygiene
 \\ \hline
         3&70403&8940&vaccines
\\ \hline 4&94149&11564&holidays, traveling \\
\hline

    \end{tabular}
   \label{tab:communities}    
\end{table}
%%to do: adjust height
 


% \subsection{Node Similarity} 
% \indent Node similarity quantifies the semantic similarity of concepts in a graph by using the underlying structure. We compute node similarity in hopes of finding hidden and nuanced relationships between COVID-related concepts. The social network of tweets at the center of our graph lets us classify and group concepts based on how they are discussed on Twitter; analyzing which concepts are frequently mentioned together, how these concepts relate to real-world events, and they evolve over time. As such, we can gain insight into opinion formation and the flow of information on social media. While there are many methods to quantify semantic similarity described in \cite{Zhu2017}, we use a random walk process. \\ \begin{figure}[!h]
% \centerline{\includegraphics[width=0.5\textwidth]{Neo4j.png}}
% \caption{Neo4j visualization for the subgraph with all entities reachable from the user with id 18003712 (red node at the center). Cypher command: \texttt{MATCH (s:User {id:`18003712'})-[*]->(t) RETURN s,t}.}
% \label{fig:neo4j}
% \end{figure}
% \subsubsection{Markov Chain Random Walk}
% \indent The underlying assumption of node similarity is that nodes with short paths between them through the social network are similar because they are mentioned together on Twitter. Nodes with many short paths between them reflect that they are mentioned together often, and are thus more similar than nodes with a fewer number of greater length. As a result, we use a Markov-chain model introduced by \cite{Fouss2007} to compute similarities. For this, we view the knowledge base as a weighted undirected graph.  \\ 
% \indent To measure the similarity between distinct nodes $i$ and $k$, we compute the \textit{average first-passage time} (AFPT): the average number of steps that a random walker will take to enter state $k$ for the first time assuming he starts in state $i\neq k$. We let $w_{ij}= w_{ji}>0$ be the weight of the edge connecting node $i$ and $j$, which represents the plausibility and importance of the link between these two nodes and is component $a_{ji}$ of the adjacency matrix $\textbf{A}$. This metric has the desired property of decreasing when the number of paths connecting two nodes increases and when the length of these paths decreases. \\ 
% % \indent Let $s(t)$ be a random variable reflecting the state of the Markov chain at time $t$, i.e. if the random walker is in state $i$ at time $t$, $s(t)=i$. The random walk is then defined by the transition probability from node $i = s(t)$ to $j = s(t+1)$: 
% % \begin{equation}
% %     P(s(t+1)= j|s(t) = i) = \frac{a_{ij}}{a_i} = p_{ij}
% %     \label{}
% % \end{equation}
% % where $a_{ij}$ is the entry of column $i$ and row $j$ in adjacency matrix $\textbf{A}$ and $a_i = \sum_{j=1}^n a_{ij}$. We can then define the recurrence relations for computing the average first-passage time $m(k|i)$ as 
% % \begin{equation}
% %     m(k|i) = 1 + \sum_{j=1}^np_{ij}m(k|j), \quad \text{for } i \neq k
% %     \label{eq:m}
% % \end{equation}
% \indent As shown in \cite{Fouss2007}, for a weighted undirected graph with $n$ vertices and adjacency matrix $\textbf{A}$, we can compute the AFPT in terms of the Moore-Penrose psuedoinverse $\textbf{L}^+$ of the Laplacian matrix $\textbf{L}$. We define the Laplacian as $\textbf{L} = \textbf{D} - \textbf{A}$, where $\textbf{D} = \text{diag}(a_i)$ with $d_{ii} = a_i = \sum_{j=1}^{n} a_{ij}$. Then we compute the AFPT from node $k$ to node $i$ as
% \begin{equation}
%     m(k|i) = \sum_{j=1}^n \left(l_{ij}^+ - l_{ik}^+ - l_{kj}^+ +  l_{kk}^+\right)d_{jj}
% \end{equation}
% where $l_{ij}^+$ is the element in row $i$, column $j$ of $\textbf{L}^+$. We use the AFPT to define a score that indicates the similarity of two nodes in the undirected graph, where a low score indicates high similarity. 
% \subsubsection{Diffusion State Distance}
% \indent To address the computational cost of approximating $\textbf{L}^+$, we implement the methods of \cite{Lin2018}, using diffusion state distance (DSD) to approximate the random walk process. We initialize a random Gaussian matrix $\textbf{Q} \in \R^{k\times n}$. The dimension $k$ is determined by the parameters $\epsilon$ and $\beta$ and is defined as 
% \begin{equation}
%     k \geq \frac{4 + 2\beta}{\epsilon^2/2 - \epsilon^3/3}\log(n)
% \end{equation}
% Introducing these parameters reduces computational cost by shrinking the dimension of the matrices used in computation. By increasing the parameter $\epsilon$ we can reduce the space complexity and memory usage of our computation, sacrificing some accuracy in the approximation. This is an important step given the high dimension of $\textbf{A}$ and $\textbf{D}$. Then, based on the Johnson-Lindenstrauss lemma outlined in \cite{Lin2018}, we compute $\widetilde{\textbf{X}} = \textbf{Q}\textbf{X} = \textbf{Q} \textbf{D}^{\frac{1}{2}}\textbf{L}\textbf{D}^{-\frac{1}{2}}$ to approximate DSD as 
% \begin{equation}
%     \widetilde{\text{DSD}}(i,j) = \norm{\widetilde{\textbf{X}}(\textbf{e}_i - \textbf{e}_j)}
% \end{equation} 
% where $\textbf{e}_i$ is the eigenvector of $\widetilde{\textbf{X}}$ associated with eigenvalue $\lambda_i$. We use the algorithm introduced in \cite{Lin2018} to compute $\tilde{\textbf{X}}$ and then calculate an approximation of DSD which we use as the node similarity score between node $i$ and $j$ in the graph. \\ 
% \indent At the time of writing, we are still analysing results and investigating ways to improve accuracy. The authors plan to pursue the idea further in hopes of shedding light on subtle connections between COVID-19 concepts in social media. 

\begin{figure*}[h!]
\includegraphics[width=0.8\textwidth]{Topic76_LP.png}
\centering
\caption{Topic 75, about social distancing. Changepoint detection shown as black lines for the initial algorithm and red lines for the graph embedding.}
\label{fig:predchange75}
\end{figure*}


\subsection{Link Prediction}
Link prediction is the process of using a graph embedding and its scoring function to predict true relations that are not explicitly in the graph. We used an embedding to predict links for the “has\_changepoint” relationships from topics to dates in an attempt to predict sentiment changepoints. 

\subsubsection{Embedding Model}


To perform link prediction, we present a new method for embedding weighted graphs. The main idea is to embed entities and relations of a knowledge graph into continuous vector spaces while preserving the underlying structure. 
%Embeddings enable a wide range of tasks, such as link prediction, triplet classification, and relation extraction. Two surveys of embedding techniques and applications are presented in \cite{Goyal2018} and \cite{Wang2017}. \\ 
Embedding a knowledge graph is a supervised learning task that represents entities and relations as vectors and defines a scoring function on each fact to measure its plausibility. We learn an embedding by minimizing the score of observed facts and maximizing the score of \textit{negative facts}, triplets that do not appear in the knowledge base. A typical knowledge graph embedding technique consists of three steps: (i) initializing entity and relation vectors, (ii) defining a scoring function, and (iii) learning an optimal relation and entity embedding. 

We adapt a translational distance model TransD \cite{Ji2015}, measuring the plausibility of a fact as the distance between two entities after some translation is carried out by a relation. TransD uses dynamic mapping matrices to translate embeddings from the entity space to the relation space. TransD is well-suited for embedding multi-relational graphs with many types of relations and entities, so it is a good fit for our graph. For example, by defining relation-specific vector spaces for each relation, our TransD embedding reflects the semantic difference between \textit{has\_keyword} and \textit{occured\_on} relations.

We begin by defining entity and relation vector spaces $\mathbb{E}\in \R^n$ and $\mathbb{P}\in \R^m$, with dimension $n$ and $m$, respectively. Given a golden triplet $\xi = (h,t,r)\in \Delta$, we define embedding vectors $\mathbf{h}, \mathbf{h}_p, \mathbf{t},\mathbf{t}_p \in \R^n$ and $\mathbf{r}, \mathbf{r}_p \R^m$, where $\cdot_p$ represents a projection vector. For each triplet $\xi $ we define two mapping matrices $\textbf{M}_{rh}, \textbf{M}_{rt} \in \R^{mxn}$ given by 
\begin{equation}
    \textbf{M}_{rh} = \textbf{r}_p\textbf{h}_p^\top + \textbf{I}^{m\times n},
    \quad
    \textbf{M}_{rt} = \textbf{r}_p\textbf{t}_p^\top + \textbf{I}^{m\times n},
    \label{eq:Mrt}
\end{equation}
which project entities from the entity space to the relation space. We then use these mapping matrices to compute the projected vectors as 
\begin{equation}
    \textbf{h}_\bot = \textbf{M}_{rh}\textbf{h}, \quad \textbf{t}_\bot = \textbf{M}_{rt}\textbf{t}.
    \label{eq:e-perp}
\end{equation}
The entity projection vectors are defined in terms of the mapping matrices, specific to the relation type. This ensures that a fact with relation $r$ is embedded into a vector space unique to that relation. An illustration of the translation via (\ref{eq:e-perp}) is shown in Fig.~\ref{fig:TransD}\cite{Ji2015}. We then use the following scoring function that incorporates these projection vectors: 
\begin{equation}
    f_r(\textbf{h}, \textbf{t}) = - \norm{\textbf{h}_\bot + \textbf{r} - \textbf{t}_\bot}_2^2
    \label{eq:TransD-score}
\end{equation}

\begin{figure*}[h!]
\includegraphics[width=0.8\textwidth]{Topic_49_Predicted_Changepoints.png}
\centering
\caption{Topic 49, about hygiene products. Change point detection shown as black lines for the initial algorithm and red lines for the graph embedding.}
\label{fig:predchange49}
\end{figure*}

\begin{figure}
\centering
\includegraphics[width=80mm]{TransD.png}

\caption{Illustration of translation step in TransD mapping facts $(\textbf{h}, \textbf{t}, \textbf{r})$ from the entity space to the relation space via matrices $\textbf{M}_{rh}$ and $\textbf{M}_{rt}$ \cite{Ji2015}}.
\label{fig:TransD} 
\end{figure}


\subsubsection{Incorporating Numeric Edge Weights}

Conventional translational embedding models embed only the facts in the knowledge base and ignore auxiliary information like node attributes and edge weights. We modify the conventional TransD scoring layer to incorporate edge weights into the embedding by combining it with a recently developed technique called FocusE, first introduced in \cite{Pai2021}, which improves the predictive abilities of our embedding. To our knowledge, we are the first group to combine TransD with FocusE. \\ 
\indent FocusE is an add-on layer in the learning cycle that is inserted between the scoring and loss layers and can be used with many conventional knowledge graph embedding models. The fundamental assumption it makes is that a numeric edge weight between two nodes represents the \textit{plausibility} that a link between them exists. This fits our graph because tweet-to-keyword, tweet-to-topic and keyword-to-topic relations have weights that are proportional to the degree to which these entities are related. \\
\indent We now extend our definition of a golden triplet to include this numeric edge weight, given by $\Delta = \{(h,t,r,w)\} \subset E \times E \times R \times \R$, where $w \in [0,1]$. Consider the TransD scoring function defined in (\ref{eq:TransD-score}). We first impose a softplus non-linearity $\sigma$ to ensure the values returned by $f_r$ are nonnegative: 
\begin{equation}
    g_r(\textbf{h}, \textbf{t}) = \sigma(f_r(\textbf{h}, \textbf{t})) = \ln(1+e^{f_r(\textbf{h}, \textbf{t})})
    \label{eq:softplus}
\end{equation}
Next, we introduce a modulating factor $\alpha \in \R$ to incorporate the numeric edge weight $w$ for a given triplet $\xi$. Defined as 
\begin{equation}
    \alpha = 
    \begin{cases*}
    \beta + (1-w)(1-\beta) \quad \text{if } \xi \in \Delta\\
    \beta + w(1-\beta) \quad \quad \quad \space \space \text{if } \xi \notin \Delta
    \end{cases*}
    \label{eq:alpha}
\end{equation}
where $\beta \in [0,1]$ measures the structural influence of the graph and is used to re-weight the triplet based on its edge weight. With $\beta = 1$ the edge weight $w$ is ignored and the model performs as a conventional embedding model. When $\beta = 0$ the edge weight is used without any modulating factor. Defining $\alpha$ in this way allows is to find a balance between the underlying structure of the graph and the influence of numeric edge weights. The FocusE layer is then defined as 
%\begin{equation}
$h_r(\textbf{h}, \textbf{t}) = \alpha\cdot g_r(\textbf{h}, \textbf{t})$
%\label{eq:h}
%\end{equation}
\indent Incorporating these numeric edge weights is especially important in our graph because the links between topics, keywords and tweets are defined by external models, and are best estimates for the presence of a link between these entities. The introduction of the FocusE layer in our model allows us to reflect the uncertainty and variability of these models, acknowledging that they are not perfect links.
\subsubsection{Training the Embedding}
\indent We first split our set of positive triplets $\Delta$ into training and validation sets, with a 95\% to 5\% split. We adopt the methods of \cite{Wang2014} to generate the set of negative triplets $\Delta'$ by Bernoulli Negative Sampling, whose parameters are based on the number of head entities per tail entity for each relation $r$. We corrupt a positive triplet $\xi$ to obtain a corresponding negative triplet $\xi'$ by replacing either the head or tail entity. Through this sampling method, each positive triplet has a corresponding negative triplet used to compute the loss function, which we seek to minimize as the training objective: 
\begin{equation}
    L = \sum_{\xi \in \Delta} \sum_{\xi' \in \Delta'} \left[\gamma + h_r(\xi') - h_r(\xi\right)]_+
    \label{eq:L}
\end{equation}
where $h_r(\textbf{h}_\bot, \textbf{t}_\bot) = h_r(\xi)$ and $h_r(\textbf{h}_\bot', \textbf{t}_\bot') = h_r(\xi')$ and $\gamma$ is a hyperparameter that represents the margin of separation between a positive and negative triplet. Our model is trained on 15 epochs with batch size of 1024 with this training objective. 

\subsubsection{Results}

In our tests, we considered any triplet with a scoring function value in the lowest 2 percent of values for its corresponding topic to suggest a link.

Our model performed quite well at predicting changepoints in sentiment trend for topics. Figure \ref{fig:predchange75} shows original and predicted sentiment changepoints for Topic 75, on social distancing. Most of the predicted changepoints line up closely with major developments in social distancing rules or other significant related events. Figure \ref{fig:predchange49} similarly shows the original and predicted changepoints for Topic 49, on hygiene products such as hand sanitizer and toilet paper. Other topics also showed promising results. This lends credibility to our NMF topics as accurately capturing timely discussion topics.

==> UCLA REU KG 10 Pages Report/conclusion.tex <==
% \section{Future Work and Applications}
% We present ideas that are interesting avenues for future work. 

% \subsection{Event Extraction using Independent Component Analysis (ICA)}
% The paper \cite{ica} runs ICA on the tweet-hashtag distribution matrix to extract real-world events and related information such as time, location, and parties involved. While the results presented in it look promising, we had little success in applying the same approach to our dataset, likely due to the low quality (and amount) of hashtags in our dataset. Running ICA on the TF-IDF matrix also gave unsatisfactory results. We still consider ICA a useful tool and would like to extract events from tweets directly without prior knowledge of actual events. The transient topics from NCPD are a good start, as they correspond well to actual events (while using the tweets as the sole source of information). However, the topics are few in number and do not contain all information needed to characterize an event (e.g. location). Future work in this area could yield more knowledge about real-world events.

% \subsection{Subgraph Matching}
% Given a template graph and a world graph, subgraph matching aims to find subgraphs of the world graph that are isomorphic (or nearly isomorphic) to the template \cite{sgmatching}. In knowledge graphs, we can additionally match types and attributes of entities and relations. If we can find interesting patterns in our knowledge graph, we can use subgraph matching to find similar patterns at other places in the graph. For example, if we can find a template characterizing the source of misinformation, we can use subgraph matching in our knowledge graph to identify possible sources of misinformation. In the future, we would need to find a way to identify interesting templates. 

% \subsection{Triple Classification}
% We can use the knowledge graph embedding to calculate the likelihood that a given triple $(h,t,r)$ is valid. Such data could have various applications, like misinformation detection.

% \subsection{Node Similarity}
% Node similarity quantifies the semantic similarity of concepts in a graph by using the underlying structure. We can quantify semantic similarity using the technique described in \cite{Zhu2017}, which uses a random walk \cite{Fouss2007}. We would compute node similarity defined in \cite{Lin2018} to find hidden and nuanced relationships between COVID-related concepts. The social network of tweets at the center of our graph lets us classify and group concepts based on how they are discussed on Twitter; analyzing which concepts are frequently mentioned together, how these concepts relate to real-world events, and they evolve over time. As such, we can gain insight into opinion formation and the flow of information on social media. 


\section{Conclusion}
In this project, we constructed and analyzed a knowledge graph of COVID-related tweets. Preprocessing and NLP summarize information into meaningful topics and allow for time series analysis. The graph structure has detectable communities, a measure of similarity between entities, allows for link prediction. Such a graph structure may allow us to answer questions of real-world importance, such as correlations between Twitter sentiment, policy changes, and spread of COVID-19; relationships between topics; clusters of tweets and/or users; and identification of misinformation.

\section*{Acknowledgments} We thank Deanna Needell and Thomas Tu for helpful conversations.

  The U.S.  Government is authorized to reproduce and distribute reprints for Governmental purposes notwithstanding any copyright notation thereon. The views and  conclusions contained herein are  those of the authors and should  not  be interpreted as necessarily representing the official policies  or endorsements, either expressed or implied, of the Air Force Research Laboratory and DARPA or the U.S. Government.


==> UCLA REU KG 10 Pages Report/construction.tex <==
\section{Graph Construction}

\indent We combine the results from our topic modeling and word embedding models with the Twitter dataset and other external information to build the knowledge graph. It represents both complex interactions in Twitter space and the important attributes of the COVID-19 pandemic around which conversation revolves. The graph is designed to simplify analyzing and understanding the interactions between the public, federal and local policymakers and the coronavirus pandemic. %In this section, we explore the structure and properties of our knowledge graph.

\subsection{Relations and Entities}

\indent The knowledge graph $G$ consists of seven entity types denoted by the set $E$ and 11 relation types denoted by the set $R$, which are summarized in Figure \ref{fig:KG structure}. Seven of these relations are defined by interactions and attributes in Twitter, and the remaining four are defined by the NLP models defined in Section III. We also present the general structure of our knowledge graph in Figure \ref{fig:KG structure}, where relations with an asterisk denote weighted edge attributes. The edge weight $w$ of a triplet $(h,t,r)$, where $h, t\in E$ and $r\in R$, intuitively represents the plausibility of a fact and may be thought of as the \textit{strength} of the connection between two entities.\\ 
\indent At the center of the knowledge graph is a social network of tweets derived from our original dataset. By connecting tweets by their interactions on Twitter we can represent the flow of information: this is useful in understanding how COVID-19 discourse is shaped by external influences and the ways in which concepts are related within the Twitter domain. We incorporate both information extracted from NLP techniques and temporal and event data to better understand the interaction between social media, real-world events, and the spread of COVID-19. Entities like topics and keywords allow us to cluster tweets based on their semantic similarity and shared concepts. Also, hashtags and users as independent entity types encode important aspects of interaction in the social media space. This lets us further group tweets and users by similar interests and conversation topics, providing useful insight into communities, concepts, and their relationships.  \\
\indent The event and date entities incorporate external knowledge and temporal information into the graph.  Including this information gives us insight into how social media conversation and real-world events interact. In addition, we store information about the spread of the coronavirus, such as case count, new cases, death count and new deaths, as an attribute of each date entity. We can analyze many of these metrics over time, which lends itself to an examination of the evolution of sentiment, ideas and concepts over the course of the coronavirus pandemic through time series analysis, change point detection algorithms and node similarity computation. Organizing a wide-range of information from social media, public policy and disease spread into a knowledge base can be used to shed light on many over arching social scientific questions and inform policy making. 
\begin{table}[!htbp]
\centering
\caption{Graph Statistics}
\resizebox{0.485\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
Relations   & Entities  & Tweets    & Users    & Hashtags & Topics & Keywords & Events & Dates \\ \hline
$5,215,237$ & $733,222$ & $635,383$ & $91,479$ & $2,540$  & $100$  & $2,000$  & $366$  & $465$ \\ \hline
\end{tabular}%
}
\label{tab:graphstat}
\end{table}

\begin{figure}
%\centering
%{.2\textwidth}
\includegraphics[width=0.5\linewidth]{WCC_size_new.png}\includegraphics[width=0.5\linewidth]{WCC_path_new.png}
\caption{(left) Distribution of sizes of weakly connected components in the tweet subgraph. Average: 1.076; Max: 126. (right) Distribution of longest path lengths of weakly connected
components in the tweet subgraph.  Average: 1.070; Max: 14.}
\label{fig:wcc_size}
\end{figure}

\subsubsection{Graph Statistics}
Table \ref{tab:graphstat} presents the numbers of relations, entities, and each type of entity in our knowledge graph. The knowledge graph contains sufficiently many relations so that it is weakly connected (i.e. we get a connected graph if we ignore edge direction); however, this is far from the case for the subgraph of all tweets. Fig. \ref{fig:wcc_size} shows the distribution of sizes (i.e. number of entities) and longest path lengths (the number of nodes in the longest path) in each of the $590,560$ weakly connected components of the subgraph. 

==> UCLA REU KG 10 Pages Report/embedding.tex <==
\section{Graph Embedding}
\indent Although knowledge graphs are effective in representing intricate networks of information, the symbolic nature of facts makes certain operations difficult. To aid this task, we introduce a knowledge graph embedding model. \\ 

\subsection{Embedding Model}
\indent The main idea of the model is to embed entities and relations of a knowledge graph into continuous vector spaces while preserving the underlying structure. Embeddings enable a wide range of tasks, such as link prediction, triplet classification, and relation extraction. Two surveys of embedding techniques and applications are presented in \cite{Goyal2018} and \cite{Wang2017}. \\ 
\indent Embedding a knowledge graph is a supervised learning task that represents entities and relations as vectors and defines a scoring function on each fact to measure its plausibility. We learn an embedding by minimizing the score of observed facts and maximizing the score of \textit{negative facts}, triplets that do not appear in our knowledge base. A typical knowledge graph embedding technique consists of three steps: (i) initializing entity and relation vectors, (ii) defining a scoring function, and (iii) learning an optimal relation and entity embedding. 
\subsubsection{Translational Distance Model}
\indent We employ a translational distance model, which measures the plausibility of a fact as the distance between two entities after some translation is carried out by a relation. For the model we consider a golden triplet $\xi = (h,t,r) \in \Delta$ with corresponding embeddings $\textbf{h},\textbf{t}\in \R^d$ and $\textbf{r}\in\R^d$, where $d$ is the dimension of the embedding space. For a true fact we have $\textbf{h} + \textbf{t} \approx \textbf{r}$, thus the scoring function $f_r(\textbf{h}, \textbf{t})$ is  given by 
\begin{equation}
    f_r(\textbf{h}, \textbf{t}) = - \norm{\textbf{h} + 
    \textbf{r} - \textbf{t}}_p,
    \label{eq:conv-score}
\end{equation}
The score is expected to be large if $(h,t,r)\in \Delta$ is an observed fact in the knowledge base. Some widely used translational distance models are TransE \cite{Bordes2013}, TransH \cite{Wang2014}, TransR \cite{Lin2015} and TransD \cite{Ji2015}. These models differ in the translation employed to map vectors from the entity space to the relation space and the reader is referred to \cite{Goyal2018} for an in depth discussion on the advantages and disadvantages of each model.\\
\indent The embedding technique we used was TransD, which uses dynamic mapping matrices to translate embeddings from the entity space to the relation space. TransD is well-suited for embedding multi-relational graphs with many types of relations and entities, so it is a good fit for our graph. For example, by defining relation-specific vector spaces for each relation, our TransD embedding reflects the semantic difference between \textit{has\_keyword} and \textit{occured\_on} relations.\\ 
\indent We begin by defining entity and relation vector spaces $\mathbb{E}\in \R^n$ and $\mathbb{P}\in \R^m$, with dimension $n$ and $m$, respectively. Given a golden triplet $\xi = (h,t,r)\in \Delta$, we define embedding vectors $\mathbf{h}, \mathbf{h}_p, \mathbf{t},\mathbf{t}_p \in \R^n$ and $\mathbf{r}, \mathbf{r}_p \R^m$, where $\cdot_p$ represents a projection vector. For each triplet $\xi $ we define two mapping matrices $\textbf{M}_{rh}, \textbf{M}_{rt} \in \R^{mxn}$ given by 
\begin{equation}
    \textbf{M}_{rh} = \textbf{r}_p\textbf{h}_p^\top + \textbf{I}^{m\times n}
    \label{eq:Mrh} 
\end{equation}
\begin{equation}
    \textbf{M}_{rt} = \textbf{r}_p\textbf{t}_p^\top + \textbf{I}^{m\times n},
    \label{eq:Mrt}
\end{equation}
which project entities from the entity space to the relation space. We then use these mapping matrices to compute the projected vectors as 
\begin{equation}
    \textbf{h}_\bot = \textbf{M}_{rh}\textbf{h}, \quad \textbf{t}_\bot = \textbf{M}_{rt}\textbf{t}.
    \label{eq:e-perp}
\end{equation}
The entity projection vectors are defined in terms of the mapping matrices, which are specific to the relation type. This ensures that a fact with relation $r$ is embedded onto a vector space unique to that relation. An illustration of the translation via (\ref{eq:e-perp}) is shown in Figure \ref{fig:TransD}\cite{Ji2015}. We then update the scoring function in (\ref{eq:conv-score}) to incorporate these projection vectors: 

\begin{figure}
\centering
\includegraphics[width=80mm]{TransD.png}

\caption{Illustration of translation step in TransD embedding model that maps facts $(\textbf{h}, \textbf{t}, \textbf{r})$ from the entity space to the relation space via mapping matrices $\textbf{M}_{rh}$ and $\textbf{M}_{rt}$ \cite{Ji2015}}
\label{fig:TransD} 
\end{figure}

\begin{equation}
    f_r(\textbf{h}, \textbf{t}) = - \norm{\textbf{h}_\bot + \textbf{r} - \textbf{t}_\bot}_2^2
    \label{eq:TransD-score}
\end{equation}
\subsubsection{Incorporating Numeric Edge Weights}
\indent Conventional translational embedding models embed only the facts in the knowledge base and ignore auxiliary information like node attributes and edge weights. We modify the conventional TransD scoring layer to incorporate edge weights into the embedding by combining it with a recently developed technique called FocusE, first introduced in \cite{Pai2021}, which improves the predictive abilities of our embedding. To our knowledge, we are the first group to combine TransD with FocusE. \\ 
\indent FocusE is an add-on layer in the learning cycle that is inserted between the scoring and loss layers and can be used with many conventional knowledge graph embedding models. The fundamental assumption it makes is that a numeric edge weight between two nodes represents the \textit{plausibility} that a link between them exists. This fits our graph because tweet-to-keyword, tweet-to-topic and keyword-to-topic relations have weights that are proportional to the degree to which these entities are related. \\
\indent We now extend our definition of a golden triplet to include this numeric edge weight, given by $\Delta = \{(h,t,r,w)\} \subset E \times E \times R \times \R$, where $w \in [0,1]$. Consider the TransD scoring function defined in (\ref{eq:TransD-score}). We first impose a softplus non-linearity $\sigma$ to ensure the values returned by $f_r$ are nonnegative: 
\begin{equation}
    g_r(\textbf{h}, \textbf{t}) = \sigma(f_r(\textbf{h}, \textbf{t})) = \ln(1+e^{f_r(\textbf{h}, \textbf{t})})
    \label{eq:softplus}
\end{equation}
Next, we introduce a modulating factor $\alpha \in \R$ to incorporate the numeric edge weight $w$ for a given triplet $\xi$. Defined as 
\begin{equation}
    \alpha = 
    \begin{cases*}
    \beta + (1-w)(1-\beta) \quad \text{if } \xi \in \Delta\\
    \beta + w(1-\beta) \quad \quad \quad \space \space \text{if } \xi \notin \Delta
    \end{cases*}
    \label{eq:alpha}
\end{equation}
where $\beta \in [0,1]$ measures the structural influence of the graph and is used to re-weight the triplet based on its edge weight. With $\beta = 1$ the edge weight $w$ is ignored and the model performs as a conventional embedding model. When $\beta = 0$ the edge weight is used without any modulating factor. Defining $\alpha$ in this way allows is to find a balance between the underlying structure of the graph and the influence of numeric edge weights. The FocusE layer is then defined as 
\begin{equation}
h_r(\textbf{h}, \textbf{t}) = \alpha\cdot g_r(\textbf{h}, \textbf{t})
\label{eq:h}
\end{equation}
\indent Incorporating these numeric edge weights is especially important in our graph because the links between topics, keywords and tweets are defined by external models, and are best estimates for the presence of a link between these entities. The introduction of the FocusE layer in our model allows us to reflect the uncertainty and variability of these models, acknowledging that they are not perfect links.
\subsection{Training the Embedding}
\indent We first split our set of positive triplets $\Delta$ into training and validation sets, with a 95\% to 5\% split. We adopt the methods of \cite{Wang2014} to generate the set of negative triplets $\Delta'$ by Bernoulli Negative Sampling, whose parameters are based on the number of head entities per tail entity for each relation $r$. We corrupt a positive triplet $\xi$ to obtain a corresponding negative triplet $\xi'$ by replacing either the head or tail entity. Through this sampling method, each positive triplet has a corresponding negative triplet used to compute the loss function, which we seek to minimize as the training objective: 
\begin{equation}
    L = \sum_{\xi \in \Delta} \sum_{\xi' \in \Delta'} \left[\gamma + g_r(\xi') - g_r(\xi\right)]_+
    \label{eq:L}
\end{equation}
where $g_r(\textbf{h}_\bot, \textbf{t}_\bot) = g_r(\xi)$ and $g_r(\textbf{h}_\bot', \textbf{t}_\bot') = g_r(\xi')$ and $\gamma$ is a hyperparameter that represents the margin of separation between a positive and negative triplet. Our model is trained on 15 epochs with batch size of 1024 with this training objective. 

\begin{figure*}[h!]
\includegraphics[width=0.8\textwidth]{Topic76 LP.png}
\centering
\caption{Changepoints for Topic 75, about social distancing. Black lines represent changepoints detected by the initial algorithm and red lines represent changepoints predicted by the graph embedding.}
\label{fig:predchange75}
\end{figure*}

\begin{figure*}[h!]
\includegraphics[width=0.8\textwidth]{Topic 49 Predicted Changepoints.png}
\centering
\caption{Changepoints for Topic 49, about hygiene products. Black lines represent changepoints detected by the initial algorithm and red lines represent changepoints predicted by the graph embedding.}
\label{fig:predchange49}
\end{figure*}


\subsection{Link Prediction}
Link prediction is the process of using a graph embedding and its scoring function to predict true facts that are not explicitly in the graph. We used our embedding to predict links for the the “associated\_with” relationship from keywords to topics and the “has\_changepoint” relationships from topics to dates. In our tests, we considered any triplet with a scoring function value in the lowest 2 percent of values for its corresponding topic to suggest a link.

\subsubsection{Identifying Keyword-Topic Associations}
We tried to apply link prediction to keyword-topic associations to expand our understanding of what subjects topics might cover and find connections between topics. Unfortunately, results for the “associated\_with” relation were underwhelming. Most words suggested by link prediction were nonsensical and had no conceivable relationship with the topic at hand. Also, there were no instances where many words associated with one topic by NMF modeling were predicted to be associated with another topic by link prediction.

\subsubsection{Identifying Changepoints}
Our model performed quite well at predicting changepoints in sentiment trend for topics. Figure \ref{fig:predchange75} shows original and predicted sentiment changepoints for Topic 75, which was about social distancing. As the image shows, most of the predicted changepoints line up closely with major developments in social distancing rules or other significant related events. Figure \ref{fig:predchange49} similarly shows the original and predicted changepoints for Topic 49, which was about hygiene products like hand sanitizer and toilet paper. Other topics also showed promising results. This lends credibility to our NMF topics as accurately capturing discussion topics.

==> UCLA REU KG 10 Pages Report/introduction.tex <==
\section{Introduction}
The past decade has seen a rapid increase in Knowledge Graph construction and analysis \st{in the literature} due to its vast industrial and academic applications. \todo[inline]{Add citations for example applications} \st{Underlying these developments is the central idea of using graphs to represent data and enhancing the representation of this data by encoding knowledge into the structure. Through encoding objects and the relationships between them in an organized structure, knowledge graphs are useful in managing, extracting and deducing information from diverse sources of data.} Knowledge graphs have many unique strengths over other methods of representing data, allowing researchers to analyze relations between data, manipulate and expand the database with ease, and quickly perform navigational operations. \st{As such, knowledge graphs have many practical uses and are employed extensively in industrial settings.} The most notable of these applications is the Google Knowledge Graph \cite{Singhal}\st{ in 2012, which marked the introduction of the idea and promoted the data model's popularity in information sciences and technology. Since then, knowledge graphs have served as a constantly evolving underlying layer of knowledge within public communities. Some} \textcolor{red}{Other} notable examples are DBpedia\cite{Lehmann}, Freebase \cite{Bollacker2007}, Wikidata \cite{Vrande2014} and YAGO \cite{Suchanek}, which are open source databases that organize large amounts of public data. 

\todo[inline]{Maybe combine this with the previous paragraph}Knowledge graphs utilize a directed graph structure to store information and encode knowledge. Nodes in the graph represent objects and often store auxiliary attributes about the object it represents, and edges represent relations between objects. This directed edge-labelled graph conforms to a graph-based data model, and can be employed for deductive and inductive tasks. Furthermore, various embedding techniques can be implemented to quantitatively represent the structure in vector space, which lends itself to semantic analysis, knowledge classification and conventional graph learning methods. For a detailed description of the common knowledge graph practices, applications and techniques, the reader is referred to \cite{Hogan2020} and \cite{Ji2020}.

\todo[inline]{What I like I doing is structuring the introduction as follows. First paragraph sets the general context, the second paragraph introduces the issue with the current approach/work that we want to address. The third paragraph then talks about what we did to address this issue.}

\todo[inline]{I think we need a paragraph in here about something that missing/wrong with current approaches. Maybe as Andrea mentioned there aren't good publicly available knowledge graphs. Or maybe we want to focus more on the covid part, and say there isnt a knowledge graph for covid that can used for ... but ours can or something}

\todo[inline]{This is now going into what we did}The knowledge graph presented in this paper outlines the construction and analysis of a COVID-19 knowledge graph with many applications. The goal of the graph is to accurately model the interaction between news developments, public opinion patterns and the spread of the virus. Through combining social media data, federal and state policy, and disease statistics into the same data structure, we can analyze the relationship between these three entities and effectively draw deductive conclusions. Moreover, we employ natural language processing techniques on social media data to enrich the information stored in the structure, enabling comparison and classification of social media interactions. The construction and analysis of the graph is broken up into four parts, which are outlined in Figure \ref{fig:process}: (1) filtering and cleaning the dataset, (2) extracting entities and relations through various natural language processing techniques, (3) constructing, visualizing and embedding, and (4) analysing the graph to deduce knowledge. At the center of the knowledge graph is an underlying social network of tweets, which models the flow of conversation on the Twitter platform. Surrounding the social network are is auxiliary information extracted from the social media data, classifications obtained through natural language processing and real-world data. We present the general structure of the graph in Figure \ref{fig:KG structure}, and explain the methods of construction and analysis in the following sections. 


\begin{figure*}
    \centering
    \includegraphics[width = 12cm]{KG Construction-updated.png}
    \caption{General structure of knowledge graph with an underlying social network of tweets at the center and external information and tweet attributes surrounding the network, where dashed edges indicate an edge weighting $w$. The tweet, hashtag and user entities are objects on extracted from Twitter; and the topic and keyword entities are generated by the NMF topic model. Event entities are complied from various news sources and reflect local and federal COVID-19 policy announcements, guideline updates, case count milestones and vaccination news. Each day spanned by the dataset is represented as a date entity.}
    \label{fig:KG structure}
\end{figure*}

\subsection{Motivation}
\todo[inline]{This needs to be earlier}
Since the onset of the novel coronavirus pandemic, researchers from a breadth of academic disciplines have been interested in tracking the interaction between developments in the crisis and social media use. Knowledge graphs are well-suited this task because they can accurately represent the content of social media data and news announcements while preserving the underlying structure of the social network and the relationships between entities. The graph also lends itself to information extraction, community detection and knowledge classification. Through constructing a database that encodes these interactions, we hope our graph can be used to shed light on how public policy announcements surrounding COVID-19 are received by the public, and how this impacts the spread of the disease. More specifically, our research is motivated by the following social scientific questions. Can we extract major coronavirus-related topics and uncover nuanced relationships between them? What is the interaction between world events, COVID-19 guideline announcements and Twitter sentiment? How does sentiment surrounding COVID-19 evolve and how, in turn, does this correlate to the spread of the disease? Can we meaningfully cluster topics, users, tweets and keywords? And, what insight can this provide about public opinion in social media?\\ 
\indent In tune with the recent influx of academic publications surrounding COVID-19, many knowledge graph techniques have been employed to better understand the pandemic and social media behavior. One of note is presented in \cite{Dimitrov2020}, which uses COVID-19 related Twitter data to construct an open source semantically annotated knowledge graph, TweetsCOV19. While the graph presented in this paper is partially motivated by the Tweets COV19 graph, we extend this model to include natural language modelling classifications, temporal data and real-world events. Additionally, our knowledge base encompasses Twitter data up to a more recent date, reflecting more recent trends in virus development, such as vaccination numbers and disease variants. Additionally, there are knowledge graphs are used in the literature to represent and analyze trends in academic research related to the coronavirus pandemic, such as \cite{Domingo2020}, \cite{Michel2020} and \cite{Wang2020}. Social media has also been a powerful tool in unravelling the dynamic spread of information, opinion and sentiment during the pandemic. Such data can be used to model Twitter discourse \cite{Wicke2021},\cite{Tsao2021}, understand public sentiment \cite{Feras2020}, \cite{Lyu2021} and perform thematic analysis\cite{Thelwall2020}. We extend and incorporate many of these ideas in the construction of our knowledge graph, combining social network analysis, COVID-19 topic analysis and knowledge base concepts to create a useful COVID-19 information model.
% Our graph differs from TweetsCOV19 in several important ways. First, the tweets in our graph are specifically from Los Angeles-related accounts. Second, our graph covers a more recent timespan than TweetsCOV19. Third, our graph captures some different information than TweetsCOV19, such as sentiment changepoints for tweet topics. Fourth, we estimate tweet sentiment using VADER, while TweetsCOV19 estimates tweet sentiment with SentiStrength. Fifth, we used a larger list of keywords when searching for COVID-related tweets than TweetsCOV19 does.



\subsection{Notation}
We define a knowledge graph as a weighted and directed edge-labelled graph $G = \{(h,t,r)\} \subset E \times E \times R$. G is a set of triples  $\xi = (h,t,r)$, $E$ is a set of entities that represent the set of nodes and $R$ is a set of relations that dictate edge labels. The graph is composed of $n = |E|$ vertices and $|R|$ relation types. We denote a set of positive facts as $\xi\in \Delta$, which is given by the triplet $(h,t,r)\in \Delta$ with corresponding edge weight $w\in \R$, where $h\in E$ and $t\in E$ are the heads and tails of a fact and $r\in R$ is the edge type that connects them. The number of edges is then enumerated by $|\Delta|$.



==> UCLA REU KG 10 Pages Report/nlp.tex <==
\section{Natural Language Processing}
%%\setcounter{tocdepth}
\begin{table*}[!h]
\centering 
\small
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}\hline 
     \textbf{Topic 1} & \textbf{Topic 2} & \textbf{Topic 6} & \textbf{Topic 8} & \textbf{Topic 9} & \textbf{Topic 10} & \textbf{Topic 11} & \textbf{Topic 14} & \textbf{Topic 17} & \textbf{Topic 19}  \\\hline 
     \cellcolor{blue!20}quarantine & \cellcolor{blue!20}mask & \cellcolor{blue!20}vaccine & \cellcolor{blue!20}test & \cellcolor{blue!20}china & \cellcolor{blue!20}symptom & \cellcolor{blue!20}case & home & \cellcolor{blue!20}trump & \cellcolor{blue!20}lockdown \\ 
     chill & wear & \cellcolor{blue!20}pfizer & positive & acre & sick & \cellcolor{blue!20}report & stay & donald & another \\ 
     self & without & dose & negative & chinese & without & \cellcolor{blue!20}number & order & \cellcolor{blue!20}administration & \cellcolor{blue!20}italy \\ 
     hair & public & shot & result & magnitude &experience & total & nursing & \cellcolor{blue!20}response & whole \\ 
     bore & \cellcolor{blue!20}mandate & second & antibody & lake & mild & confirm & send & rally & full \\
     vibe & nose & \cellcolor{blue!20}moderna & site & biden & doctor & record & leave & plan & protest \\ 
     mood & damn & appointment & player & communist & fever & update & nurse & supporter & extend \\ 
     ain & protect & recieve & rapid & russia & morning & daily & safer & election & city \\ 
     wanna & store & vaccinate & testing & america & hospital & million & patient & hoax & order \\ 
     whole & walk & available & available & blame & update & increase & workout & campaign & lift \\ \hline 
    \textbf{Topic 28} & \textbf{Topic 44} & \textbf{Topic 49} & \textbf{Topic 59} & \textbf{Topic 70} & \textbf{Topic 75} & \textbf{Topic 88} & \textbf{Topic 89} & \textbf{Topic 91} & \textbf{Topic 94}  \\\hline 
    still & \cellcolor{blue!20}healthcare & hand & watch & \cellcolor{blue!20}state & \cellcolor{blue!20}social & \cellcolor{blue!20}open & happy & \cellcolor{blue!20}president & \cellcolor{blue!20}check \\ 
    despite & \cellcolor{blue!20}worker & \cellcolor{blue!20}sanitizer & \cellcolor{blue!20}movie &united & \cellcolor{blue!20}distancing & school & birthday & \cellcolor{blue!20}biden & \cellcolor{blue!20}relief \\ 
    \cellcolor{blue!20}partying & plan & wash & video & \cellcolor{blue!20}governor & distance & \cellcolor{blue!20}close & party & vice & vote \\ 
    breaker & system & smell & netflix & mandate & practice & business & \cellcolor{blue!20}celebrate & obama & bill \\ 
    flock & essential & bottle & episode & florida & medium & read & friday & force & stimulus \\ 
    spring & molina & paper & game & magnitude & guideline & store & easter & task & pass \\ 
    miami & click & shake & katie & acre & continue & high & wish & patriotic & senate \\ 
    there & frontline & wipe & youtube & lake & follow & restaurant & thanks & penny & republican \\ 
    warning & universal & toilet & porter & federal & physical & reopen & monday & fight & package \\ 
    vaccinate & nurse & soap & holy & order & maintain & everything & weekend & former & money\\ \hline 
\end{tabular}
\caption{Top keywords for 20 selected coherent topics from the 100 topics obtained from the entire dataset using NMF. Some meaningful words are highlighted.}
\label{fig:nmf_all}
\end{table*}
In this section we discuss the natural language processing (NLP) methods used to analyze sentiment, extract topics and uncover keywords from the Twitter dataset, which are then incorporated into the knowledge graph. 

\subsection{Sentiment Analysis}
Sentiment analysis on Twitter data provides insight into the user's attitude towards a particular concept, is an integral part of knowledge graph construction, and acts as the basis for time series analysis. We quantify sentiment by calculating the sentiment score $s\in [-1,1]$, where $|s|$ indicates the sentiment intensity and the sign indicates whether the sentiment is positive or negative. We use the Valence Aware Dictionary for sEntiment Reasoning (VADER) library\cite{vader} to calculate and assign the sentiment score of each tweet's original text.

%We use aspect-based sentiment analysis (ABSA) to capture the attitude towards a given word within the context of the text in which is appears. For example, when analyzing sentences like ``I like apples but dislike pears,'' VADER would assign a single score (likely close to 0), while the sentence actually contains different sentiments towards two ``aspect words:'' ``apples'' and ``pears.'' In knowledge graph construction, we extract the aspect-based sentiment score of keywords within the context of a tweet, capturing a tweet's attitude towards a particular COVID-19 related keyword. We then store this value as a numeric edge weight for tweet-to-keyword relations.

To obtain numeric edge weights for tweet-to-keyword relations, we assign sentiment scores for each keyword contained in a tweet.  We implement an algorithm that yields aspect-based sentiment scores based on VADER. Given a tweet and a set of keywords appearing in the tweet, the algorithm performs the following steps. Note that for sentiment analysis, we do not use the cleaned text, but the raw text from the tweets. 

\begin{enumerate}[1.]
\item Divide a sentence into clauses, using punctuation and conjunctions as separators.\footnote{VADER detects sentiment from some punctuation and conjunctions, thus it is important where separators are placed. For our purposes, keep punctuation with their preceding clauses and the conjunctions with their following clauses.}
\item Use VADER to find the sentiment score of each clause.
\item For each aspect word, find clauses where the word appears, and assign the average score of all such clauses as the sentiment score of the relation.
\end{enumerate}

\subsection{Topic Modeling}
Topic modelling summarizes tweet contents, cluster tweets by topics, examine thematic trends, and perform additional time series analysis. The results are incorporated as topic entities and tweet-to-topic relations in our graph.
\newcommand{\ndocs}{m}
\newcommand{\nterms}{n}
\newcommand{\ntopics}{u}
\newcommand{\nslices}{s}
\newcommand{\ndates}{d}
We denote the number of documents by $\ndocs$, number of terms by $\nterms$, and number of topics by $\ntopics$. %; for a matrix $\matx M$, $\matx M_i$ denotes the $i$-th column of $\matx M$; and $\otimes$ denotes the outer product. 
Given a list of terms and a corpus of tweets, we first compute the term frequency-inverse document frequency (TF-IDF) matrix, representing how often each term appears in each document \cite{tfidf}. Then we apply factorization algorithms, namely Non-negative Matrix Factorization (NMF)\cite{nmf} and Non-negative Canonical Polyadic Decomposition (NCPD)\cite{ncpd1}\cite{ncpd2}, to find a small number of hidden topics, described by their distribution over documents, terms, and time. NMF gives a summary of the topics discussed over the whole dataset, while NCPD naturally analyzes these topics over time.

%\iffalse
%\subsubsection{NMF}
%NMF aims to factor a matrix into the product of two matrices with non-negative entries, as described in detail in \cite{nmf}. We used the scikit-learn, or sklearn library \cite{sklearn} to perform NMF and TF-IDF, which uses Nonnegative Double Singular Value Decomposition (NNDSVD)\cite{nndsvd} for initialization and a coordinate descent solver. 

Using the scikit-learn (sklearn) library \cite{sklearn}, we run NMF on the entire dataset with $\ntopics=100$ topics. Table \ref{fig:nmf_all} demonstrates a subset of our results, and suggests that NMF yields meaningful topics that reflect real-world events.

% \begin{figure*}[!h]
% \centerline{\includegraphics[width=0.9\textwidth]{NMF_all.png}}
% \caption{Top keywords for 20 selected coherent topics from the 100 topics obtained from the entire dataset using NMF. Some meaningful words are highlighted.}
% \label{fig:nmf_all}
% \end{figure*}



\iffalse
\subsubsection{NCPD}

As described in \cite{ncpd1}\cite{ncpd2}, NCPD takes as input a data tensor $\tnsr T\in\R^{\nslices\times\ndocs\times\nterms}$ with $\nslices$ slices. The third dimension can be thought of as a representation of time: for each $1\leq i\leq\nslices$, the slice at time $i$ is a matrix $\tnsr T_i\in\R^{m\times n}$ which is the TF-IDF matrix of all documents at time $i$. We then attempt to find matrices $\matx S\in\R^{\nslices\times\ntopics}, \matx B\in\R^{\ndocs\times\ntopics}, \matx C\in\R^{\nterms\times\ntopics}$ with non-negative entries such that the Frobenius norm \begin{equation}
    \|\tnsr T-\sum_{i=1}^r\matx A_i\otimes\matx B_i\otimes\matx C_i\|
\end{equation}is minimized. The $i$-th topic is represented by the tensor $\matx A_i\otimes\matx B_i\otimes\matx C_i$, with $\matx A_i,\matx B_i,\matx C_i$ describing its distribution over time (slices), documents, and terms, respectively. By incorporating temporal information into $\tnsr T$, NCPD allows us to track the evolution of topics over time more directly.
\fi

NCPD uses a data tensor $\tnsr T\in\R^{\nslices\times\ndocs\times\nterms}$, where the slice at time $i$ is the TF-IDF matrix $\tnsr T_i\in\R^{m\times n}$ of all documents at time $i$ for each $1\leq i\leq\nslices$. We divide the tweets into equal slices (continuous over time) and fix the vocabulary for the entire dataset to ensure each $\tnsr T_i$ has the same number of rows ($\ndocs$) and columns ($\nterms$), respectively. We use the TensorLy libary \cite{tensorly} to run NCPD on the whole dataset with $\nslices=306, \ndocs=2000, \ntopics=20$ (Fig~\ref{fig:ncpd}).   We observe some transient topics (e.g. topics 4, 5, 7, 11, and 16) that are discussed more frequently in a short period of time.

% These results indicate that NCPD demonstrates topic evolution over time better than NMF. In addition,s, as observed in \cite{ncpd}. Even though NCPD has a higher computational cost compared to NMF, it provides new insight into our dataset. 

\begin{figure*}[!h]
\centerline{\includegraphics[width=0.8\textwidth]{NCPD_label.png}}
\caption{The evolution of 20 NCPD topics over time. To improve resolution, the data was clipped to exclude March 2020 (when an extremely high peak occurred at Topic 0). The following real-world events correspond to visible peaks in the respective topics in the heatmap: (Topic 4) Donald Trump suggested injection of disinfectants in response to COVID-19 on April 24, 2020; (Topic 16) Orange county lifted mask restrictions on June 11, 2020; (Topic 7) GOP nominated Donald Trump for 2020 President Election on August 24, 2020; (Topics 5,11) Donald and Melania Trump tested positive for COVID-19 on October 2, 2020.}
\label{fig:ncpd}
\end{figure*}

\subsubsection{Results}
Overall, both topic modeling approaches provide a useful summary of the dataset. The NMF topics shown in Table \ref{fig:nmf_all} are coherent and form a foundation for further analysis. The NCPD results in Fig.~\ref{fig:ncpd} not only show the popularity of recurring topics over time, but also capture localized topics corresponding to actual events. For example, Topic 16 corresponds to Orange County lifting mask restrictions. These results connect our dataset to real-world events and enable further analysis. %These topics will represent important entities in our graph.

\subsection{Time Series Analysis}
In order to gain insight into how COVID-19 topics and social media discourse change over time, we employ time series analysis. This also lends itself to an understanding of the juxtaposition between real-world events, public opinion and disease spread.
\subsubsection{Sentiment Change Over Time}
After each tweet in the dataset is assigned a sentiment score, we group tweets by date and calculate the daily average sentiment score. We observe that sentiment around COVID-19 increases when the the COVID-19 vaccine became widely available to the public around April 2021, as shown in Fig~\ref{fig:sentiment}. 
\begin{figure*}[h!]
\includegraphics[width = 0.7\linewidth]{overall_sentiment_newest.png}
\centering
\caption{Change point detection applied to Sentiment of all tweets, grouped by dates. Recent-7-day average sentiment is calculated to decrease the noise of oscillations. Excluding the last date which is always classified as a change point, the change points are 5/24/2020, 11/05/2020, and 1/29/2021.}
\label{fig:sentiment}
\end{figure*}

\subsubsection{Peak and Change Point Detection}

\paragraph{Volume of Tweets}
We perform a soft clustering using the 100 NMF topics such that each tweet belongs to at least one topic. Then, we plot tweet volume over time for all topics and align important events with dates at which peaks occur through analyzing text and news events. 
\begin{figure*}[h!]
\includegraphics[width = 0.9\linewidth]{topic6_volume.png}
\centering
\caption{Tweet volume of topic 6 per day. There are 4 sharp peaks on 03/21/2020, 11/09/2020, 12/18/2020, 04/13/2021, respectively, from left to right.}
\label{fig:t6vol}
\end{figure*}

Figure \ref{fig:t6vol} shows the volume of tweets in topic 6, (a vaccine topic see Table~\ref{fig:nmf_all}).
%for topic keywords), over time. 
We find that peaks on 03/21/2020, 11/09/2020, 12/18/2020, 04/13/2021 correspond to considerable discussions about the development of COVID-19 vaccines: Pfizer declaring 90\% effectiveness of its vaccine, first COVID-19 vaccine administered in LA county, and the production halt of Johnson \& Johnson's vaccines, respectively. These four events are highly related to the keywords of topic 6 extracted from the NMF model. By detecting peaks in the tweet volume of each topic, we are able to identify dates when important events related to that topic take place.

\paragraph{Change Point Detection on Sentiment Change}    




\mbox{}\par 
\iffalse
Change point detection (CPD) \cite{killick} helps detect abrupt changes in time series data and transitions between states. Given an ordered sequence of data $y_{1:n} = (y_{1}, ..., y_{n})$, CPD gives ordered change points $m$ and their ordered timestamps $\tau = (\tau_{1}, ..., \tau_{m})$. Define $\tau_{0} = 0$ and $\tau_{m+1} = n$. The ordering implies $\tau_{i} < \tau_{j}$ if and only if $i < j$. The $m$ change points split the data into $m + 1$ segments, with the $i^{th}$ segment containing $y_{(\tau_{i-1}+1):\tau_{i}}.$
To identify multiple change points, we minimize the following formula:
$$\sum_{i=1}^{m+1}{C(y_{(\tau_{i-1}+1):\tau_{i}}) + \beta f(m)},$$
where $C$ is a cost function for each segment and $\beta f(m)$ is a penalty to prevent overfitting.
\fi

Change point detection (CPD) \cite{killick} helps detect abrupt changes in time series data and transitions between states, finding a number of change points $\tau = (\tau_{1}, ..., \tau_{m},\tau_{m+1}=n)$ that minimize a cost function (which measures changes) in an ordered sequence of data $y_{1:n} = (y_{1}, ..., y_{n})$. We use the Pruned Exact Linear Time (PELT)\cite{killick} to perform CPD as it maintains low computational costs while preserving accuracy. We adjusted the hyper-parameter of the penalty function as follows: First, we select a random topic and find important dates associated to that topic (using real world news data). Then we update the hyper-parameter so that the change points detected by PELT are approximate to the actual important dates and use the resulting value in the model.

We apply change point detection to the daily average sentiment data from March 11, 2020 to June 17, 2021 to investigate how the sentiment change of tweets reflect real-world events. We present CPD results of Topic 75 in Figure \ref{fig:t75}. CPD was successful in detecting important dates associated with social distancing guidelines. However, not all 100 topics have meaningful change points that relate to real-world events. We believe these results could be improved by increasing sentiment score accuracy. It is generally difficult to accurately classify the sentiment of social media language due to abbreviations, sarcasm, irony, etc. Another possibility is that our Twitter dataset may not reflect the accurate sentiment change of a specific topic because of the inadequate tweet volumes of some NMF topics and the limitation of our dataset to only the Los Angeles area. 

These change point will be important relations in our knowledge graph. Specifically, our graph has topics and dates as entities in the graph. Hence the change points will be relations connecting a topic to the date. We will shall eventually use these our graph to predict new relations of this type. 
 
\begin{figure*}[h!]
\includegraphics[width=0.9\linewidth]{topic75_cpd_updated.png}
\centering
\caption{Change point detection applied on sentiment of tweets in topic 75. Recent-7-day average sentiment is calculated to decrease the noise of oscillation. }
\label{fig:t75}
\end{figure*}

\subsection{Word Embedding}
\iffalse We implement a word embedding model to define the relation between tweets and keywords extracted from the NMF topic model. Recall that each tweet belongs to at least one NMF topic and each topic has a list of associated keywords. For each tweet we select a keyword from the associated topic keyword, such that there is a word in the tweet semantically similar to the keyword. To compare the semantic meaning of two words, we introduce word embedding. 
\fi

\iffalse
Common word embedding models translate all the words in the corpus into the same vector space, where each word is represented by a vector. Furthermore, any two words that share similar semantic meaning, or are likely to occur in the same context, should have relatively short distance between each other\cite{wordEmbedding}. The similarity between two words $a$, $b$ is defined as their cosine similarity in the vector space
\begin{equation}
    \cos(\theta) = \frac{\vctr{v_{a}}\cdot \vctr{v_{b}}}{\mathopen|\vctr{v_{a}}\mathclose|\mathopen|\vctr{v_{b}}\mathclose|}
\end{equation}, where $\vctr{v_{a}}$and $\vctr{v_{b}}$ denotes the vector representations for word $a$ and $b$, respectively. From the definition, we can see that the similarity between two words varies from $-1$ to 1 inclusively, with 1 indicating two words are exactly the same.
\fi

Word embedding models allow us to measure semantic similarity between words quantitatively as the cosine similarity of the embedded vectors. With word embedding, for each tweet we can identify a word from its text and a keyword from its associated NMF topic such that the similarity between the word and the keyword is maximized. Then we add an edge between the keyword and tweet, and use the similarity value as the edge's weight.  % find for each tweet a keyword from its associated NMF topic that is semantically similar to a word in the tweet's text, and use it to define a relation between tweet and keywords.

We use the word embedding model glove-twitter-200\cite{glove}, which is pre-trained on a corpus of common words from Twitter in 2017. We also implement Word2Vec with the Python package gensim\cite{gensim} to train another word embedding model with the words from the dataset to incorporate a more up to date and relevant dictionary. Then we combine the two models, so new words that came up after glove-twitter-200 was trained, such as "COVID-19", are also included in our model. 

==> UCLA REU KG 10 Pages Report/preprocessing.tex <==
\section{Pre-processing}
Our dataset consists of more than 7 million tweets from March 11, 2020 through June 17, 2021 authored by accounts with a geography tag in Los Angeles County and tweets geotagged within this region. 


\begin{figure*}[h!]
\centering
\includegraphics[width = 0.8\linewidth]{overview.png}
\caption{Overview of the research process used to create and analyze the knowledge graph of interest. The filtering and cleaning of data of is outlined Section II and an overview of the models used to define relationships in the structure are presented in Section III. Graph construction and analysis techniques are then explained in detail in Sections IV and V, respectively.}
\label{fig:process}
\end{figure*}

\subsection{Filtering}
 We filter the original dataset (chosen by date and location) to include tweets pertaining to the pandemic. %To do so, we construct a list of relevant keywords to filter tweets by their text content. 
 We begin with a list of 268 COVID-19 related keywords\footnote{https://data.gesis.org/tweetscov19/keywords.txt} introduced in \cite{Dimitrov2020}. To include keywords relating to more recent COVID-19 updates like vaccines, we include keywords mentioned in \cite{Deverna2021} and the keywords used to generate the COVID-19 Twitter stream.\footnote{https://developer.twitter.com/en/docs/labs/covid19-stream/filtering-rules} Combining these three lists generated a set of 467 COVID-19 related keywords to use for filtering. 
We search the text of each tweet for these keywords. If a COVID-19 related keyword appears in the text of a tweet, that tweet and all tweets that are in the reply thread of that tweet are added to the filtered dataset. 
%In addition, if a tweet is part of a reply thread that for a tweet that contains the , we search the text of other tweets within the thread for the presence of a COVID-19 related word. If the seed tweet of a reply thread (i.e. the tweet that began the reply thread) contains one of these words, we add every tweet that replied to this tweet to the filtered dataset, whether or not it contains a COVID-19 related keyword. 
This allows us to include tweets that respond and react to COVID-19 information in our filtered dataset. The resulting dataset contains 635,383 tweets from 91,443 unique users.

\subsection{Cleaning the Data}
To analyze the content of our dataset and organize the information in a useful way, we pre-process the raw data before performing topic modeling, word embedding and construction of the knowledge graph. This is important given the complex language present in social media data and is crucial in extracting meaningful information about sentiment and opinion formation. We adapt the methods of \cite{Lai2016} as follows: remove non-Alphanumeric characters, user mentions, URLs, hashtags, English and Spanish stop words, and words less than three letters long. We make all characters lowercase and then tag parts of speech and lemmatize text.
These steps rid the text of unnecessary emojis, punctuation, and auxiliary information that distract from the meaning of the tweet. We store user mentions and hashtags of tweets in separate fields of the dataframe, incorporating them in the construction of the knowledge graph. This allows us to account for important information without distracting from the language of the tweet. We import stop words from the Natural Language Toolkit (NLTK) library in Python \cite{nltk} and manually expand this set with common social media slang. We perform part-of-speech tagging and lemmatization with NLTK's \texttt{WordNetLemmatizer}, yielding an abbreviated version of the text that just contains the meaningful words in the tweet. 
%Once the text is cleaned, we export a dataframe of tweets with which we construct the knowledge graph and natural language processing models. We then use this tokenized text in our word embedding and topic models. \\
\begin{table}[htbp]
    \centering
    \caption{Tweet attributes stored in dataframe after pre-processing}
    
    \begin{tabular}{|l c p{5cm}|}
    \hline
         \textbf{Field}  & \textbf{Data type} &  \textbf{Description}\\ \hline
         tweet ID & \texttt{int} & Unique tweet identification number \newline generated by Twitter API \\ \hline
         created at & \texttt{str} & Date and time tweet was published \newline in UTC timezone \\ \hline
         user ID & \texttt{int} & Unqique user ID number of tweet author \newline generated by Twitter API \\ \hline
         text & \texttt{str} & Original, uncleaned text of tweet\\ \hline
         \newline cleaned text & \texttt{list str} & Cleaned and tokenized text of tweet \\ \hline
         hashtags & \texttt{list str} & List of hashtags in original 
         \newline text field denoted by \# prefix \\\hline
         mentions & \texttt{list str} & List of user mentions in original \newline text field denoted by @ prefix \\ \hline 
         in-reply-to & \texttt{int} & Tweet ID of original tweet in reply thread \\ \hline
         quoted & \texttt{int} & Tweet ID of tweet quoted by current tweet  \\ \hline
    \end{tabular}
    \label{tab:tweet-att}
    
\end{table}

In addition to storing the cleaned text, we retain other auxiliary information about each tweet extracted from our dataset stored in Twitter API format\footnote{https://developer.twitter.com/en/docs/twitter-api/v1/data-dictionary/object-model/tweet} to benefit knowledge graph construction and application. These attributes are summarized in Table \ref{tab:tweet-att}. With the processed text and attributes stored, we then perform various natural language processing tasks to provide insight into the text contents of our dataset. 



==> embedding.tex <==
\section{Graph Embedding}
\indent Although knowledge graphs are effective in representing intricate networks of information, the symbolic nature of facts makes certain operations difficult. To aid this task, we introduce a knowledge graph embedding model. \\ 

\subsection{Embedding Model}
\indent The main idea of the model is to embed entities and relations of a knowledge graph into continuous vector spaces while preserving the underlying structure. Embeddings enable a wide range of tasks, such as link prediction, triplet classification, and relation extraction. Two surveys of embedding techniques and applications are presented in \cite{Goyal2018} and \cite{Wang2017}. \\ 
\indent Embedding a knowledge graph is a supervised learning task that represents entities and relations as vectors and defines a scoring function on each fact to measure its plausibility. We learn an embedding by minimizing the score of observed facts and maximizing the score of \textit{negative facts}, triplets that do not appear in our knowledge base. A typical knowledge graph embedding technique consists of three steps: (i) initializing entity and relation vectors, (ii) defining a scoring function, and (iii) learning an optimal relation and entity embedding. 
\subsubsection{Translational Distance Model}
\indent We employ a translational distance model, which measures the plausibility of a fact as the distance between two entities after some translation is carried out by a relation. For the model we consider a golden triplet $\xi = (h,t,r) \in \Delta$ with corresponding embeddings $\textbf{h},\textbf{t}\in \R^d$ and $\textbf{r}\in\R^d$, where $d$ is the dimension of the embedding space. For a true fact we have $\textbf{h} + \textbf{t} \approx \textbf{r}$, thus the scoring function $f_r(\textbf{h}, \textbf{t})$ is  given by 
\begin{equation}
    f_r(\textbf{h}, \textbf{t}) = - \norm{\textbf{h} + 
    \textbf{r} - \textbf{t}}_p,
    \label{eq:conv-score}
\end{equation}
The score is expected to be large if $(h,t,r)\in \Delta$ is an observed fact in the knowledge base. Some widely used translational distance models are TransE \cite{Bordes2013}, TransH \cite{Wang2014}, TransR \cite{Lin2015} and TransD \cite{Ji2015}. These models differ in the translation employed to map vectors from the entity space to the relation space and the reader is referred to \cite{Goyal2018} for an in depth discussion on the advantages and disadvantages of each model.\\
\indent The embedding technique we used was TransD, which uses dynamic mapping matrices to translate embeddings from the entity space to the relation space. TransD is well-suited for embedding multi-relational graphs with many types of relations and entities, so it is a good fit for our graph. For example, by defining relation-specific vector spaces for each relation, our TransD embedding reflects the semantic difference between \textit{has\_keyword} and \textit{occured\_on} relations.\\ 
\indent We begin by defining entity and relation vector spaces $\mathbb{E}\in \R^n$ and $\mathbb{P}\in \R^m$, with dimension $n$ and $m$, respectively. Given a golden triplet $\xi = (h,t,r)\in \Delta$, we define embedding vectors $\mathbf{h}, \mathbf{h}_p, \mathbf{t},\mathbf{t}_p \in \R^n$ and $\mathbf{r}, \mathbf{r}_p \R^m$, where $\cdot_p$ represents a projection vector. For each triplet $\xi $ we define two mapping matrices $\textbf{M}_{rh}, \textbf{M}_{rt} \in \R^{mxn}$ given by 
\begin{equation}
    \textbf{M}_{rh} = \textbf{r}_p\textbf{h}_p^\top + \textbf{I}^{m\times n}
    \label{eq:Mrh} 
\end{equation}
\begin{equation}
    \textbf{M}_{rt} = \textbf{r}_p\textbf{t}_p^\top + \textbf{I}^{m\times n},
    \label{eq:Mrt}
\end{equation}
which project entities from the entity space to the relation space. We then use these mapping matrices to compute the projected vectors as 
\begin{equation}
    \textbf{h}_\bot = \textbf{M}_{rh}\textbf{h}, \quad \textbf{t}_\bot = \textbf{M}_{rt}\textbf{t}.
    \label{eq:e-perp}
\end{equation}
The entity projection vectors are defined in terms of the mapping matrices, which are specific to the relation type. This ensures that a fact with relation $r$ is embedded onto a vector space unique to that relation. An illustration of the translation via (\ref{eq:e-perp}) is shown in Figure \ref{fig:TransD}\cite{Ji2015}. We then update the scoring function in (\ref{eq:conv-score}) to incorporate these projection vectors: 

\begin{figure}
\centering
\includegraphics[width=80mm]{TransD.png}

\caption{Illustration of translation step in TransD embedding model that maps facts $(\textbf{h}, \textbf{t}, \textbf{r})$ from the entity space to the relation space via mapping matrices $\textbf{M}_{rh}$ and $\textbf{M}_{rt}$ \cite{Ji2015}}
\label{fig:TransD} 
\end{figure}

\begin{equation}
    f_r(\textbf{h}, \textbf{t}) = - \norm{\textbf{h}_\bot + \textbf{r} - \textbf{t}_\bot}_2^2
    \label{eq:TransD-score}
\end{equation}
\subsubsection{Incorporating Numeric Edge Weights}
\indent Conventional translational embedding models embed only the facts in the knowledge base and ignore auxiliary information like node attributes and edge weights. We modify the conventional TransD scoring layer to incorporate edge weights into the embedding by combining it with a recently developed technique called FocusE, first introduced in \cite{Pai2021}, which improves the predictive abilities of our embedding. To our knowledge, we are the first group to combine TransD with FocusE. \\ 
\indent FocusE is an add-on layer in the learning cycle that is inserted between the scoring and loss layers and can be used with many conventional knowledge graph embedding models. The fundamental assumption it makes is that a numeric edge weight between two nodes represents the \textit{plausibility} that a link between them exists. This fits our graph because tweet-to-keyword, tweet-to-topic and keyword-to-topic relations have weights that are proportional to the degree to which these entities are related. \\
\indent We now extend our definition of a golden triplet to include this numeric edge weight, given by $\Delta = \{(h,t,r,w)\} \subset E \times E \times R \times \R$, where $w \in [0,1]$. Consider the TransD scoring function defined in (\ref{eq:TransD-score}). We first impose a softplus non-linearity $\sigma$ to ensure the values returned by $f_r$ are nonnegative: 
\begin{equation}
    g_r(\textbf{h}, \textbf{t}) = \sigma(f_r(\textbf{h}, \textbf{t})) = \ln(1+e^{f_r(\textbf{h}, \textbf{t})})
    \label{eq:softplus}
\end{equation}
Next, we introduce a modulating factor $\alpha \in \R$ to incorporate the numeric edge weight $w$ for a given triplet $\xi$. Defined as 
\begin{equation}
    \alpha = 
    \begin{cases*}
    \beta + (1-w)(1-\beta) \quad \text{if } \xi \in \Delta\\
    \beta + w(1-\beta) \quad \quad \quad \space \space \text{if } \xi \notin \Delta
    \end{cases*}
    \label{eq:alpha}
\end{equation}
where $\beta \in [0,1]$ measures the structural influence of the graph and is used to re-weight the triplet based on its edge weight. With $\beta = 1$ the edge weight $w$ is ignored and the model performs as a conventional embedding model. When $\beta = 0$ the edge weight is used without any modulating factor. Defining $\alpha$ in this way allows is to find a balance between the underlying structure of the graph and the influence of numeric edge weights. The FocusE layer is then defined as 
\begin{equation}
h_r(\textbf{h}, \textbf{t}) = \alpha\cdot g_r(\textbf{h}, \textbf{t})
\label{eq:h}
\end{equation}
\indent Incorporating these numeric edge weights is especially important in our graph because the links between topics, keywords and tweets are defined by external models, and are best estimates for the presence of a link between these entities. The introduction of the FocusE layer in our model allows us to reflect the uncertainty and variability of these models, acknowledging that they are not perfect links.
\subsection{Training the Embedding}
\indent We first split our set of positive triplets $\Delta$ into training and validation sets, with a 95\% to 5\% split. We adopt the methods of \cite{Wang2014} to generate the set of negative triplets $\Delta'$ by Bernoulli Negative Sampling, whose parameters are based on the number of head entities per tail entity for each relation $r$. We corrupt a positive triplet $\xi$ to obtain a corresponding negative triplet $\xi'$ by replacing either the head or tail entity. Through this sampling method, each positive triplet has a corresponding negative triplet used to compute the loss function, which we seek to minimize as the training objective: 
\begin{equation}
    L = \sum_{\xi \in \Delta} \sum_{\xi' \in \Delta'} \left[\gamma + g_r(\xi') - g_r(\xi\right)]_+
    \label{eq:L}
\end{equation}
where $g_r(\textbf{h}_\bot, \textbf{t}_\bot) = g_r(\xi)$ and $g_r(\textbf{h}_\bot', \textbf{t}_\bot') = g_r(\xi')$ and $\gamma$ is a hyperparameter that represents the margin of separation between a positive and negative triplet. Our model is trained on 15 epochs with batch size of 1024 with this training objective. 

\begin{figure*}[h!]
\includegraphics[width=0.8\textwidth]{Topic76 LP.png}
\centering
\caption{Changepoints for Topic 75, about social distancing. Black lines represent changepoints detected by the initial algorithm and red lines represent changepoints predicted by the graph embedding.}
\label{fig:predchange75}
\end{figure*}

\begin{figure*}[h!]
\includegraphics[width=0.8\textwidth]{Topic 49 Predicted Changepoints.png}
\centering
\caption{Changepoints for Topic 49, about hygiene products. Black lines represent changepoints detected by the initial algorithm and red lines represent changepoints predicted by the graph embedding.}
\label{fig:predchange49}
\end{figure*}


\subsection{Link Prediction}
Link prediction is the process of using a graph embedding and its scoring function to predict true facts that are not explicitly in the graph. We used our embedding to predict links for the the “associated\_with” relationship from keywords to topics and the “has\_changepoint” relationships from topics to dates. In our tests, we considered any triplet with a scoring function value in the lowest 2 percent of values for its corresponding topic to suggest a link.

\subsubsection{Identifying Keyword-Topic Associations}
We tried to apply link prediction to keyword-topic associations to expand our understanding of what subjects topics might cover and find connections between topics. Unfortunately, results for the “associated\_with” relation were underwhelming. Most words suggested by link prediction were nonsensical and had no conceivable relationship with the topic at hand. Also, there were no instances where many words associated with one topic by NMF modeling were predicted to be associated with another topic by link prediction.

\subsubsection{Identifying Changepoints}
Our model performed quite well at predicting changepoints in sentiment trend for topics. Figure \ref{fig:predchange75} shows original and predicted sentiment changepoints for Topic 75, which was about social distancing. As the image shows, most of the predicted changepoints line up closely with major developments in social distancing rules or other significant related events. Figure \ref{fig:predchange49} similarly shows the original and predicted changepoints for Topic 49, which was about hygiene products like hand sanitizer and toilet paper. Other topics also showed promising results. This lends credibility to our NMF topics as accurately capturing discussion topics.

==> introduction.tex <==
\section{Introduction}
The past decade has seen a rapid increase in Knowledge Graph construction and analysis \st{in the literature} due to its vast industrial and academic applications. \todo[inline]{Add citations for example applications} \st{Underlying these developments is the central idea of using graphs to represent data and enhancing the representation of this data by encoding knowledge into the structure. Through encoding objects and the relationships between them in an organized structure, knowledge graphs are useful in managing, extracting and deducing information from diverse sources of data.} Knowledge graphs have many unique strengths over other methods of representing data, allowing researchers to analyze relations between data, manipulate and expand the database with ease, and quickly perform navigational operations. \st{As such, knowledge graphs have many practical uses and are employed extensively in industrial settings.} The most notable of these applications is the Google Knowledge Graph \cite{Singhal}\st{ in 2012, which marked the introduction of the idea and promoted the data model's popularity in information sciences and technology. Since then, knowledge graphs have served as a constantly evolving underlying layer of knowledge within public communities. Some} \textcolor{red}{Other} notable examples are DBpedia\cite{Lehmann}, Freebase \cite{Bollacker2007}, Wikidata \cite{Vrande2014} and YAGO \cite{Suchanek}, which are open source databases that organize large amounts of public data. 

\todo[inline]{Maybe combine this with the previous paragraph}Knowledge graphs utilize a directed graph structure to store information and encode knowledge. Nodes in the graph represent objects and often store auxiliary attributes about the object it represents, and edges represent relations between objects. This directed edge-labelled graph conforms to a graph-based data model, and can be employed for deductive and inductive tasks. Furthermore, various embedding techniques can be implemented to quantitatively represent the structure in vector space, which lends itself to semantic analysis, knowledge classification and conventional graph learning methods. For a detailed description of the common knowledge graph practices, applications and techniques, the reader is referred to \cite{Hogan2020} and \cite{Ji2020}.

\todo[inline]{What I like I doing is structuring the introduction as follows. First paragraph sets the general context, the second paragraph introduces the issue with the current approach/work that we want to address. The third paragraph then talks about what we did to address this issue.}

\todo[inline]{I think we need a paragraph in here about something that missing/wrong with current approaches. Maybe as Andrea mentioned there aren't good publicly available knowledge graphs. Or maybe we want to focus more on the covid part, and say there isnt a knowledge graph for covid that can used for ... but ours can or something}

\todo[inline]{This is now going into what we did}The knowledge graph presented in this paper outlines the construction and analysis of a COVID-19 knowledge graph with many applications. The goal of the graph is to accurately model the interaction between news developments, public opinion patterns and the spread of the virus. Through combining social media data, federal and state policy, and disease statistics into the same data structure, we can analyze the relationship between these three entities and effectively draw deductive conclusions. Moreover, we employ natural language processing techniques on social media data to enrich the information stored in the structure, enabling comparison and classification of social media interactions. The construction and analysis of the graph is broken up into four parts, which are outlined in Figure \ref{fig:process}: (1) filtering and cleaning the dataset, (2) extracting entities and relations through various natural language processing techniques, (3) constructing, visualizing and embedding, and (4) analysing the graph to deduce knowledge. At the center of the knowledge graph is an underlying social network of tweets, which models the flow of conversation on the Twitter platform. Surrounding the social network are is auxiliary information extracted from the social media data, classifications obtained through natural language processing and real-world data. We present the general structure of the graph in Figure \ref{fig:KG structure}, and explain the methods of construction and analysis in the following sections. 


\begin{figure*}
    \centering
    \includegraphics[width = 12cm]{KG Construction-updated.png}
    \caption{General structure of knowledge graph with an underlying social network of tweets at the center and external information and tweet attributes surrounding the network, where dashed edges indicate an edge weighting $w$. The tweet, hashtag and user entities are objects on extracted from Twitter; and the topic and keyword entities are generated by the NMF topic model. Event entities are complied from various news sources and reflect local and federal COVID-19 policy announcements, guideline updates, case count milestones and vaccination news. Each day spanned by the dataset is represented as a date entity.}
    \label{fig:KG structure}
\end{figure*}

\subsection{Motivation}
\todo[inline]{This needs to be earlier}
Since the onset of the novel coronavirus pandemic, researchers from a breadth of academic disciplines have been interested in tracking the interaction between developments in the crisis and social media use. Knowledge graphs are well-suited this task because they can accurately represent the content of social media data and news announcements while preserving the underlying structure of the social network and the relationships between entities. The graph also lends itself to information extraction, community detection and knowledge classification. Through constructing a database that encodes these interactions, we hope our graph can be used to shed light on how public policy announcements surrounding COVID-19 are received by the public, and how this impacts the spread of the disease. More specifically, our research is motivated by the following social scientific questions. Can we extract major coronavirus-related topics and uncover nuanced relationships between them? What is the interaction between world events, COVID-19 guideline announcements and Twitter sentiment? How does sentiment surrounding COVID-19 evolve and how, in turn, does this correlate to the spread of the disease? Can we meaningfully cluster topics, users, tweets and keywords? And, what insight can this provide about public opinion in social media?\\ 
\indent In tune with the recent influx of academic publications surrounding COVID-19, many knowledge graph techniques have been employed to better understand the pandemic and social media behavior. One of note is presented in \cite{Dimitrov2020}, which uses COVID-19 related Twitter data to construct an open source semantically annotated knowledge graph, TweetsCOV19. While the graph presented in this paper is partially motivated by the Tweets COV19 graph, we extend this model to include natural language modelling classifications, temporal data and real-world events. Additionally, our knowledge base encompasses Twitter data up to a more recent date, reflecting more recent trends in virus development, such as vaccination numbers and disease variants. Additionally, there are knowledge graphs are used in the literature to represent and analyze trends in academic research related to the coronavirus pandemic, such as \cite{Domingo2020}, \cite{Michel2020} and \cite{Wang2020}. Social media has also been a powerful tool in unravelling the dynamic spread of information, opinion and sentiment during the pandemic. Such data can be used to model Twitter discourse \cite{Wicke2021},\cite{Tsao2021}, understand public sentiment \cite{Feras2020}, \cite{Lyu2021} and perform thematic analysis\cite{Thelwall2020}. We extend and incorporate many of these ideas in the construction of our knowledge graph, combining social network analysis, COVID-19 topic analysis and knowledge base concepts to create a useful COVID-19 information model.
% Our graph differs from TweetsCOV19 in several important ways. First, the tweets in our graph are specifically from Los Angeles-related accounts. Second, our graph covers a more recent timespan than TweetsCOV19. Third, our graph captures some different information than TweetsCOV19, such as sentiment changepoints for tweet topics. Fourth, we estimate tweet sentiment using VADER, while TweetsCOV19 estimates tweet sentiment with SentiStrength. Fifth, we used a larger list of keywords when searching for COVID-related tweets than TweetsCOV19 does.



\subsection{Notation}
We define a knowledge graph as a weighted and directed edge-labelled graph $G = \{(h,t,r)\} \subset E \times E \times R$. G is a set of triples  $\xi = (h,t,r)$, $E$ is a set of entities that represent the set of nodes and $R$ is a set of relations that dictate edge labels. The graph is composed of $n = |E|$ vertices and $|R|$ relation types. We denote a set of positive facts as $\xi\in \Delta$, which is given by the triplet $(h,t,r)\in \Delta$ with corresponding edge weight $w\in \R$, where $h\in E$ and $t\in E$ are the heads and tails of a fact and $r\in R$ is the edge type that connects them. The number of edges is then enumerated by $|\Delta|$.


